LATE Ain'T Earley: A Faster Parallel Earley Parser

We present the LATE algorithm, an asynchronous variant of the Earley algorithm for parsing context-free grammars. The Earley algorithm is naturally task-based, but is difficult to parallelize because of dependencies between the tasks. We present the LATE algorithm, which uses additional data structures to maintain information about the state of the parse so that work items may be processed in any order. This property allows the LATE algorithm to be sped up using task parallelism. We show that the LATE algorithm can achieve a 120x speedup over the Earley algorithm on a natural language task.

==> algorithm.tex <==
\section{Algorithm}

In this section we discuss the Earley algorithm, starting with the standard
serial implementation and a naive parallelization. We then present LATE, a novel parsing algorithm created by augmenting the Earley algorithm with additional data structures to allow for asynchronous execution of Earley tasks.

%In this section we will discuss the Earley algorithm, starting with the standard
%serial implementation (Section~\ref{sec:serial}). Next, we will describe a
%scheme for parallelizing the Earley algorithm which uses speculation about the
%contents of the Earley sets to achieve parallelism (Section~\ref{sec:parallel}).
%Finally, we will describe an automata based scheme for optimizing the serial
%Earley algorithm and consider how automata can be used to improve the parallel
%Earley algorithm: in particular, how automata may help with the problems caused
%by speculation (Section~\ref{sec:automata}).

\subsection{Serial Earley Parsing}\label{sec:serial}

The Earley algorithm~\cite{earley_efficient_1970} is a type of chart parser. It
constructs a data structure which contains all of the parses of the input
sentence. The data structure consists of sets of \emph{Earley items}. An Earley
item represents a partial parse of a rule of the form $S \rightarrow \alpha
\dots$, where $S$ is the nonterminal produced from the terminals $\alpha
\dots$. We will refer to a position $p$ as the space between the $p^{th}$
symbol and the $(p + 1)^{th}$ symbol in the input sentence. The Earley items
each contain an origin position $i$ which represents the location where the
rule started parsing. They also contain a current position $k$ which represents
the current parse location of the rule in the input. The Earley items use a
$\bullet$ to represent the current parse position within the rule itself.  Thus,
the Earley rule $S \to \alpha \bullet \beta$ at origin $i$ and current position
$k$ represents a partial parse of the nonterminal $S$ using input symbols from
positions $i$ to $k$, where $\alpha$ has already been parsed and we have yet to
parse $\beta$. We will write an Earley item as $(S \to \alpha \bullet \beta, i,
k)$, or when $k$ is clear from the context we may abbreviate as $(S \to \alpha
\bullet \beta, i)$.

The Earley chart is a data structure which stores a sets of Earley items for
each input position.  The Earley set $k$ consists of all Earley items with
current input position $k$. The Earley algorithm uses the START rule to
initialize the chart (Lines~\ref{ln:init-start}-\ref{ln:init-end}). The main
loop iterates through the chart and applies one of three subroutines for each
new item added to a set: the predictor, the scanner, and the completer.

The scanner runs on unfinished rules whose next symbol (the symbol after the
$\bullet$) is a terminal $T$. If the string contains this symbol in position $k$,
the scanner advances the rule and puts it in the next Earley set
(Lines~\ref{ln:scan-start}-\ref{ln:scan-end}). This advancing of rules is
analogous to the shift action in an LR parser.

The predictor runs on unfinished rules whose next symbol is a non-terminal $N$.
For these rules to advance, $N$ needs to be parseable. The predictor inserts all
of the grammar rules which can parse $N$ into the current Earley set
(Lines~\ref{ln:pred-start}-\ref{ln:pred-end}).

The completer runs on finished Earley items, where the entire right hand side
of the rule has been parsed. If the rule is finished, then we have seen a
successful parse of the nonterminal on the left hand side, and we need to
advance rules that were waiting on these parses.  When it finds a finished rule
$S \rightarrow \alpha \bullet$, the completer returns to the Earley set where the
rule originated. Any rule that has $S$ as its next symbol to parse can be
advanced, so the completer puts them in the current item set
(Lines~\ref{ln:cmp-start}-\ref{ln:cmp-end}). The operation of the completer is
analogous to the reduce action in an LR parser.

\subsection{Parallel Earley Parsing}\label{sec:parallel}

A simple approach to parallelizing the Earley algorithm runs the inner loop
(Lines~\ref{ln:inner-start}-\ref{ln:inner-end}) using several worker threads,
treating the set of Earley items like a work queue. Unfortunately, it is
difficult to make this parallel processing efficient, because we need to ensure
that each thread does enough work to balance the overhead of distributing the
work between threads. The Earley sets are often small, meaning that there is
little parallel work. When we investigated this technique, we found that the
parallel overhead is greater than the speedup from parallelism, so there is no
performance benefit.

\subsection{LATE Parsing}
\label{sec:late}

  Earley parsing is difficult to parallelize because we cannot run the
completer on a finished Earley item originating at position $i$ and producing
some symbol $S$ until we have added all of the items at current position $i$
that will use $S$ as their next symbol. If we process our finished item too
early, the items that use $S$ as their next symbol will not be processed since
the predict step cannot advance rules.  This limitation forces the processing
order of the Earley items in increasing order of current location.

  This same limitation complicates Earley parsing of $\epsilon$ symbols (which
represent empty strings). Suppose we are about to use the Earley algorithm to
process the item $(S \to \bullet \alpha \alpha, i, k)$ and that there exists a
rule $\alpha \to \epsilon$. Prediction adds $(\alpha \to \bullet \epsilon, k, k)$
to the chart, then scanning adds $(\alpha \to \epsilon \bullet, k, k)$.
Completion of $(\alpha \to \epsilon \bullet, k, k)$ advances the original item
once, adding $(S \to \alpha \bullet \alpha, i, k)$ to the chart, but prediction
on $(S \to \alpha \bullet \alpha, i, k)$ will only add $(\alpha \to \bullet
\epsilon, k, k)$, which has been added before.  Since the predict step cannot
advance rules, $(S \to \alpha \bullet \alpha, i, k)$ will never be advanced
again.

  There are special purpose fixes for the case of processing $\epsilon$
correctly, but we can actually solve both of these problems at the same time in
a more general way by adding three new data structures that allow the predict
step to advance Earley items. We call our modified algorithm the LATE
algorithm. The LATE parser produces the same chart as the Earley Parser, but
tasks can be completed in parallel.

  The Earley parser stores a chart for each input position $k$ filled with
items of the form $(\dots, i)$.  For simplicity, the LATE parser stores a
global chart (line \ref{ln:late-chart}) with items of the form $(\dots, i, k)$.
The LATE parser also stores three additional data structures, the
\emph{requests} map, the \emph{replies} map, and the \emph{completed} set. When
the predict step processes a state $(S \to \dots \bullet N \dots, i, k)$, we say
that the nonterminal symbol $N$ has been requested at input position $k$ by
this state.  The requests data structure (line \ref{ln:late-requests}) maps from
a tuple $(N, k)$ of a requested symbol and the input position where it has been
requested to a list of states which requested this symbol at this location.
When the parse of a symbol is completed, we say that this is a reply to the
request. The replies data structure (line \ref{ln:late-replies}) maps from a
tuple $(N, i)$ of a requested symbol and the input position where it has been
requested to a list of input positions where the requested symbol has been
parsed starting at $i$ and ending at $k$. To avoid redundant complete
operations, the completed set (line \ref{ln:late-completed}) stores tuples $(N,
i, k)$ of completed parses of nonterminals $N$ originating at position $i$ and
ending at position $k$.

  Like the Earley parser, the Late parser only processes states once. The scan
step is the same as in the Earley algorithm.

  The LATE predict step now adds its state to the requests data structure, and
adds advanced copies of this state to each position in the replies
data structure. If no requests have yet been made for a nonterminal, then all
rules which can parse the nonterminal are added to the current position.

  The LATE complete step first checks if its completed parse of a symbol is in
the completed set. If it is, the complete step can stop early. Otherwise, the
symbol, origin, and current position tuple is added to the completed set. Next,
we add the current (finished) location to the replies list at the origin of the
completed symbol, then advance all states in the requests list at the origin of
the completed symbol to the current position.

\begin{figure}
\hspace{-0.125\textwidth}%
\begin{minipage}[t]{0.6\textwidth}
  \vspace{0pt}
  \begin{algorithm}[H]
  \input{alg_earley}
  \caption{The serial Earley algorithm for parsing
    CFGs~\cite{earley_efficient_1970}.}
  \label{alg:earley}
\end{algorithm}
\end{minipage}%
\hspace{0.05\textwidth}%
\begin{minipage}[t]{0.6\textwidth}
    \vspace{0pt}
  \begin{algorithm}[H]
    \input{alg_late}
    \caption{The serial LATE algorithm for parsing CFGs.}
    \label{alg:late}
  \end{algorithm}
\end{minipage}%
\hspace{-0.125\textwidth}%
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> progress.tex <==
\section{Progress To Date}

To date we have implemented three versions of the Earley parser: a Python
implementation, a sequential C++ implementation, and a parallel C++
implementation that uses task threading to achieve parallelism. At this point,
our parallel implementation is not faster than our sequential version. We
believe that this is because our parallel version performs work in chunks that
are too small, so the gains of parallelism are eaten up by the overhead of
distributing the work.

As discussed in Section~\ref{sec:parallel}, a successful parallel Earley parser
breaks its work into blocks that can be computed mostly independently, so our
future implementations will focus on ensuring that we break the necessary work
into larger chunks.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

